Next-to-leading order QCD corrections to Higgs production at a future lepton-proton collider

Crucial information on the coupling of the Higgs boson to bottom quarks is expected from Higgs production in association with a forward tagging jet at a future high-energy lepton-proton collider. In order to control the theoretical uncertainties of the signal process, the impact of radiative corrections has to be quantified. We present the full next-to-leading order QCD corrections to e- p -> e- j H and e- p -> nu_e j H in the form of a flexible Monte-Carlo program allowing for the calculation of cross sections and kinematic distributions within experimentally feasible selection cuts. QCD corrections are found to be very small for cross sections, while the shape distortion of distributions can be as large as 20%. Residual scale uncertainties at next-to-leading order are at the permille level.

==> setup.tex <==
\usepackage{graphics}
%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{cite}
\usepackage{eufrak}
\usepackage{rotating}
\usepackage{wasysym}

\hfuzz .5pt

\makeatletter
 \setlength{\clubpenalty}{10000}
 \setlength{\widowpenalty}{10000}
 \setlength{\displaywidowpenalty}{10000}

\arraycolsep 2pt
\footnotesep 14pt

\if@twoside \oddsidemargin -17pt \evensidemargin 00pt
\else \oddsidemargin 00pt \evensidemargin 00pt
\fi
\topmargin 00pt \headheight 00pt \headsep 00pt
\textheight 230mm \textwidth 161mm

\renewcommand{\theparagraph}{(\roman{paragraph})}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{+2.00ex plus
 +1ex minus +.2ex}{1.5ex plus .2ex}{\it\normalsize}}

\expandafter\ifx\csname mathrm\endcsname\relax\def\mathrm#1{{\rm #1}}\fi

% Equation Numbering
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\newcounter{saveeqn}
\newcommand{\alpheqn}{\setcounter{saveeqn}{\value{equation}}%
   \addtocounter{saveeqn}{1} \setcounter{equation}{0}%
   \renewcommand{\theequation}%
   {{\thesection.\arabic{saveeqn}\alph{equation}}}}
\newcommand{\reseteqn}{\setcounter{equation}{\value{saveeqn}}%
   \renewcommand{\theequation}{\thesection.\arabic{equation}}}
 
\@addtoreset{equation}{section}

\makeatother

\renewcommand{\topfraction}{0.7}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.2}
\renewcommand{\floatpagefraction}{0.7}

% new commands
\def\REF#1#2{\\[-4cm] \hspace*{#1} \rlap{\vphantom{\rule{1mm}{4cm}}
        \parbox[b]{16cm}{\baselineskip 16pt{\normalsize #2}}}}
\def\co{\relax}
\def\co{,}
\def\nl{\nonumber\\}
\def\nlc{\co\nonumber\\}
\def\nln{\nonumber\\*[-1ex]\phantom{\fbox{\rule{0em}{2ex}}}}
\def\eqskipcorr{\vspace{-\abovedisplayskip}
                \vspace{\abovedisplayshortskip}}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\bec{\begin{center}}
\def\eec{\end{center}}

\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\non}{\nonumber}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\mr}{\mathrm}
\newcommand{\hs}{\hspace*}
\newcommand{\vs}{\vspace*}

\def\dec{d}
\def\muf{\mu_\mr{F}}
\def\mur{\mu_\mr{R}}
\def\cc{eq\to~\nu_e\, q' H}
\def\nc{eq\to~e q H}
\def\ccp{ep\to~\nu_e\, j H}
\def\ncp{ep\to~e\, j H}
\def\eps{\varepsilon}
\def\lq{\left[} 
\def\rq{\right]} 
\def\rg{\right\}} 
\def\lg{\left\{} 
\def\({\left(} 
\def\){\right)} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



